Automated, Cost-effective, and Update-driven App Testing

Apps' pervasive role in our society led to the definition of test automation approaches to ensure their dependability. However, state-of-the-art approaches tend to generate large numbers of test inputs and are unlikely to achieve more than 50% method coverage. In this paper, we propose a strategy to achieve significantly higher coverage of the code affected by updates with a much smaller number of test inputs, thus alleviating the test oracle problem. More specifically, we present ATUA, a model-based approach that synthesizes App models with static analysis, integrates a dynamically-refined state abstraction function and combines complementary testing strategies, including (1) coverage of the model structure, (2) coverage of the App code, (3) random exploration, and (4) coverage of dependencies identified through information retrieval. Its model-based strategy enables ATUA to generate a small set of inputs that exercise only the code affected by the updates. In turn, this makes common test oracle solutions more cost-effective as they tend to involve human effort. A large empirical evaluation, conducted with 72 App versions belonging to nine popular Android Apps, has shown that ATUA is more effective and less effort intensive than state-of-the-art approaches when testing App updates.

==> approach_CICD.tex <==


\subsection{Integrating \APPR into CI/CD practices}
\label{sec:approach:cicd}

Figure~\ref{fig:process:lifecycle} shows how \APPR can be used to test an App during its lifecycle. 
It is first used to test the initial version of the App (i.e., V0 in Figure~\ref{fig:process:lifecycle}).
For the initial version, every method of the App is considered to be a test target.
For every following version, \APPR considers only updated methods as test targets. 

We rely on Figure~\ref{fig:process:lifecycle} to exemplify how \APPR reaches its objectives, i.e., (O1) minimize the number of methods that need to be manually tested for every App version, and (O2) automatically exercise most of the App methods over the App lifecycle.

Figure~\ref{fig:process:lifecycle}, exemplifies the differences in coverage that can be observed when comparing \APPR (Letter \emph{A}) with a state-of-the-art approach (Letter \emph{S}). In Figure~\ref{fig:process:lifecycle}, we assume that the test budget enables both the state-of-the-art approach and \APPR to exercise only three methods. 
The methods that are not exercised by automated test cases need to be exercised through manual testing. 
In the case of state-of-the-art approaches, engineers will need to manually exercise at least seven methods through the lifecycle of the App: methods \emph{d()} and \emph{e()} for \emph{V0}, methods \emph{e()} and \emph{f()} for \emph{V1}, method \emph{g()} for \emph{V2}, methods \emph{g()} and \emph{h()} for \emph{V3}.
In the case of \APPR, instead, engineers will have to manually test only methods \emph{d()} and \emph{e()} for \emph{V0}, which shows that \APPR is a better choice to achieve both O1 and O2. Section~\ref{sec:empirical} provides empirical evidence.


\APPR can be easily integrated into CI/CD practices, by automating its execution overnight, weekly, or before a public release of the App.




\begin{figure}[t]
  \centering
	\includegraphics{images/AutAutLifecycle}
      \caption{Overview of the \APPR{} process to test App updates.}
      \label{fig:process:lifecycle}
\end{figure}



==> approach_Instrument.tex <==

\subsection{Step 3. Instrument the App Under Test}
\label{sec:approach:Instrument}


==> data/RQ2_ALL_1Hour_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex <==

1&24.18/16.19/32.35
\\

2&40.95/22.01/49.66
\\

3&16.53/13.54/20.37
\\

4&4.54/-5.96/11.32
\\

5&19.64/14.56/24.55
\\

6&35.97/25.30/46.09
\\

7&4.45/-1.59/10.73
\\

8&26.69/9.00/34.55
\\

9&13.11/11.19/16.21
\\



==> data/RQ2_ALL_5Hours_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex <==

1&32.83/30.33/39.29
\\

2&38.85/28.46/44.83
\\

3&20.95/18.57/23.47
\\

4&10.17/4.77/17.92
\\

5&11.52/-0.84/28.82
\\

6&32.56/28.02/35.94
\\

7&26.52/20.37/33.64
\\

8&31.01/19.85/40.60
\\

9&21.27/13.83/25.42
\\



==> data/RQ2_SameActionBudget_ALL_1Hour_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex <==

1&17.99/7.83/26.69
\\

2&20.06/3.17/34.66
\\

3&2.70/-1.37/6.36
\\

4&13.01/1.33/20.26
\\

5&16.04/10.02/21.59
\\

6&18.66/6.47/39.66
\\

7&11.41/-2.90/19.90
\\

8&2.47/-10.06/7.96
\\

9&3.47/-1.32/23.60
\\



==> data/RQ2_SameActionBudget_ALL_5Hours_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex <==

1&12.36/6.23/18.57
\\

2&30.44/15.94/43.96
\\

3&6.12/1.87/13.32
\\

4&8.34/0.08/16.65
\\

5&6.27/-3.63/23.13
\\

6&14.98/-3.70/39.51
\\

7&0.62/-5.84/5.25
\\

8&8.57/-1.62/17.20
\\

9&5.38/-6.52/15.66
\\



==> evaluation_RQ2_2.tex <==

\subsection{RQ2.2: Effectiveness within Time Budget  (Whole-App)}

\subsubsection{Experiment design}

\CHANGED{\APPR targets App updates and, as a result, we need to investigate if it is also effective for testing the first version of the App under test.  \CHANGEDNOV{Indeed, \APPR works by exercising target Windows and Abstract States according to a priority order. For  the first version of an App, all the methods and instructions  should be tested and  thus the prioritized strategy implemented by \APPR might perform worse than a random strategy.} However, since \APPR implements a model-based approach that integrates information retrieval, static analysis, and a state abstraction function that relies on dynamic analysis, we aim to study if \APPR can nevertheless outperform state-of-the-art approaches when the entire App should be tested.}

To address RQ2, we measure the percentage of methods and instructions belonging to the first version of each subject App (i.e., V0) that are automatically exercised by test automation tools.
To positively answer this research question, \APPR should, in statistical terms, achieve higher coverage than the other approaches.


\subsubsection{Results}

Figures~\ref{fig:RQ3:MethCoveredV0:1} to~\ref{fig:RQ3:InstrCoveredV0:5} show, for each subject App, the percentage of methods and instructions that are automatically tested by the different approaches with one-hour and five-hour execution time budgets. 



With a one-hour budget, \APPR achieves the highest percentage of methods and instructions being exercised on average, with \FIXME{48.27\%} and \FIXME{44.83\%}, respectively.
The largest differences are observed when \APPR is compared to Monkey; indeed, on average, \APPR exercises \FIXME{23.37\%} and \FIXME{21.20\%} more methods and instructions than Monkey, respectively. 
\APPR exercises \FIXME{13.62\%} and \FIXME{12.49\%} more target methods and instructions than APE, respectively.
Finally, \APPR exercises \FIXME{3.96\%} and \FIXME{4.56\%} more target methods and instructions than DM2. 


\input{tables/effectSizeRQ22.tex}

Table~\ref{table:effectSize:rq22} shows the Mann Whitney U-test p-value and $A_{12}$ statistics. For both method and instruction coverage, differences are significant except for 4 out of 27 cases. With ActivityDiary (subject App 2) and File Manager (case 3), \APPR exercises less methods than DM2; however, for File Manager, there is no significant difference between \APPR and DM2 in terms of instruction coverage. 
DM2 and \APPR  do not show significant differences also for method coverage in the case of 
VLC player (case 8). 



With a test budget of five hours, all the approaches achieve slightly better coverage results; however, the ranking observed for a one-hour budget remains unchanged.
\APPR is the approach with the average highest percentage of exercised target methods and instructions, with \FIXME{51.14\%} and \FIXME{47.51\%}, respectively.
The second-best approach is still DM2, which exercises \FIXME{2.95\%} and \FIXME{3.38\%} fewer target methods and instructions than \APPR. 

A larger time budget enables \APPR to fare better than DM2 in the case of Activity Diary and File Manager ($A_{12} > 0.80$). In the case of YahooWeather (case 5), DM2 and Monkey perform better than \APPR ($A_{12} < 0.30$), while APE performs better than \APPR for Wikipedia (case 1),  ActivityDiary (case 2), and Wikihow (case 6). DM2 and \APPR fare similarly in the case of BBC Mobile. In these cases, 
\CHANGEDNOV{since any method of the App should be tested,}
\CHANGEDNOV{approaches based on random exploration
that do not integrate analyses aiming at reaching specific updated features (e.g., \APPR target Windows)
can benefit from the time saved to exercise a larger number of methods/instructions.} \APPR, instead, is limited by static analysis, which often identifies a superset of the feasible paths to reach target Windows (see Section~\ref{sec:algo}); consequently, \APPR wastes part of its test budget in exploring paths that cannot reach target Windows. In addition, both DM2 and \APPR show performance limitations in the presence of WebViews, which are instead properly processed by APE; indeed, APEwhich outperforms both \APPR and DM2 in the case of Wikipedia (case 1) and Wikihow (case 6), two Apps highly relying on WebViews.

\CHANGEDNOV{To summarize, on average, \APPR performs better than the other approaches for both test budgets. For an execution time of one hour, \APPR remains the favorable choice since it outperforms the other approaches for eight out of nine subject Apps and is comparable to DM2 for one case only. 
For an execution time of five hours, \APPR still performs better than other approaches for the majority of the cases, i.e., five out of nine subject Apps. However, when a large test budget is available, the characteristic of the App under test might drive the choice of the testing tool. For example, APE might be an optimal choice when the App largely relies on WebViews.
In general, our results show that the strategies integrated by \APPR not only facilitate the testing of App updates but also enable effective testing of the entire App.
}


\begin{figure*}
\centering
\begin{minipage}{.45\textwidth}
  \centering
	\includegraphics[width=8.5cm]{data/RQ3_SameActionBudget_ALL_1Hour_COMPARISON_modifiedMethodsCoverageFirst}
      \caption{Percentage of methods of the first App versions that are  covered for each subject App (budget=1 hour).}
      \label{fig:RQ3:MethCoveredV0:1}
\end{minipage}\hspace{10mm}
\begin{minipage}{.45\textwidth}
  \centering
	\includegraphics[width=8.5cm]{data/RQ3_SameActionBudget_ALL_5Hours_COMPARISON_modifiedMethodsCoverageFirst}
      \caption{Percentage of methods of the first App versions that are covered for each subject App (budget=5 hours).}
      \label{fig:RQ3:MethCoveredV0:5}
\end{minipage}
\begin{minipage}{.45\textwidth}
  \centering
	\includegraphics[width=8.5cm]{data/RQ3_SameActionBudget_ALL_1Hour_COMPARISON_modifiedInstructionsCoverageFirst}
      \caption{Percentage of instructions of the first App versions that are  covered for each subject App (budget=1 hour).}
      \label{fig:RQ3:InstrCoveredV0:1}
\end{minipage}\hspace{10mm}
\begin{minipage}{.45\textwidth}
  \centering
	\includegraphics[width=8.5cm]{data/RQ3_SameActionBudget_ALL_5Hours_COMPARISON_modifiedInstructionsCoverageFirst}
      \caption{Percentage of instructions of the first App versions that are covered for each subject App (budget=5 hours).}
      \label{fig:RQ3:InstrCoveredV0:5}
\end{minipage}
\end{figure*}

\CHANGEDNOV{\subsection*{Threats to validity}}

To address threats to external validity we have considered nine popular Apps, downloaded thousands of times worldwide, that had been considered in the empirical evaluation of related work. Also, for each App, we considered up to ten App versions, based on their availability, for a total of 81 App versions tested. 
The considered Apps vary for number of lines of code and for the number of lines of code updated between versions. Because of their diversity, we believe our subject Apps to be representative of Apps market.

To account for randomness, we tested each App version ten times with every testing tool considered; more than the usual practice of three to five repetitions~\cite{}. This enabled us to derive solid statistics for the comparison of  different tools.

In our experiments we considered only Android Apps, which is standard practice in most App testing research papers. This enabled comparison of \APPR with tools working with Android Apps only (i.e., Monkey, APE, and DM2). Since we do not exercise OS-specific features, results should generalize also to Apps running in different execution environments (e.g., HarmonyOS and IOS).









==> oldRQ2.tex <==

\subsection{RQ2: Test effort over lifecycle}

\subsubsection{Experiment design}

A surrogate measure of the effort required to test an App over its lifecycle is the overall number of instructions belonging to updated methods that are not covered by automated testing. Indeed, engineers have to manually implement test cases that exercise these instructions. Therefore, for all the case study Apps, we identify all the instructions belonging to the updated methods of versions V0 to V9 that that need to be tested manually. 
For a given test automation tool $T$ and an App $A$, we measure the effort required to test $A$ over its lifecycle as the sum of the number of instructions that need to be tested manually in the i-th run according to the formula
$\mathit{effort}_{T,A,i}=\sum_{v=\mathit{V1}}^{\mathit{VL}}{\mathit{missing}_{T}(v)}$,
where $\mathit{missing}(v)$ is the number of instructions not covered by the test automation tool $T$ for version $v$, and VL is the last available version for the App A (usually V9).

For each subject of the study, we measure, in percentage points, the effort reduction of \AutAut with respect to another test automation approach $O$, according to the formula
$$\mathit{reduction}_{O,i}=\frac{\mathit{effort}_{O}-\mathit{effort}_{\APPR}}{\mathit{effort}_{O}}*100$$

We inspect the distribution of the effort reduction for the different approaches and case study systems. To positively answer our research question, the effort reduction should be always positive and significant.



\subsubsection{Results}

Figures~\ref{fig:RQ2:InstrNotCovered:1} and ~\ref{fig:RQ2:InstrNotCovered:5} show, for each case study, the percentage of instructions that should be manually tested, when a certain test automation tools is used. \APPR achieves the best results since the median and the average number of instructions to be manually tested is below the one obtained by the other techniques.

Table~\ref{table:RQ2} shows the effort reduction of \AutAut with respect to the other test automation approaches. In general, \AutAut shows a positive reduction, which indicates that \APPR is a better  choice to test Apps in their lifecycle. Further, \APPR performs better than other approaches with a larger test execution budget as well, thus suggesting that the generated models enable an optimal use of the test budget.

\begin{figure}[t]
  \centering
	\includegraphics[width=8.5cm]{data/RQ2_1Hour_COMPARISON_instructions_NotCovered_over_lifecycle}
      \caption{Percentage of instructions that need to be manually tested for each subject of the study (budget=1 hour).}
      \label{fig:RQ2:InstrNotCovered:1}
\end{figure}

\begin{figure}[t]
  \centering
	\includegraphics[width=8.5cm]{data/RQ2_5Hours_COMPARISON_instructions_NotCovered_over_lifecycle}
      \caption{Percentage of instructions that need to be manually tested for each subject of the study (budget=5 hours).}
      \label{fig:RQ2:InstrNotCovered:5}
\end{figure}

\input{tables/RQ2.tex}








==> tables/RQ2.tex <==

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{2cm}|p{3cm}|}
\hline
\textbf{Case}&\multicolumn{1}{|c|}{\textbf{Effort Reduction (avg/min/max)}}\\
\textbf{study}&\multicolumn{1}{|c|}{\textbf{wrt DM2}}\\
\hline
\input{data/RQ2_1Hour_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex}
\hline
\input{data/RQ2_5Hours_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex}
\hline
\end{tabular}
\caption{Effort reduction with respect to other approaches. Top part shows results with budget of one hour, bottom part shows results for five hours.}
\label{table:RQ2}
\end{table}%


==> tables/effectSizeRQ22.tex <==



\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for RQ2.2.}
\label{table:effectSize:rq22}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
}
\hline
\textbf{}&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{C}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
&
\multicolumn{12}{c|}{\textbf{Coverage of target methods}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.890&1.00&.890
&<0.05&<0.05&<0.05&.640&.820&\R{.320}\\
2&<0.05&<0.05&<0.05&\R{.370}&.990&.850
&<0.05&<0.05&<0.05&.890&1.00&1.00\\
3&\R{0.80}&<0.05&<0.05&\R{.350}&1.00&.900
&\R{0.46}&<0.05&0.99&.845&.975&.600\\
4&<0.05&<0.05&<0.05&.960&1.00&.950
&<0.05&<0.05&<0.05&.950&1.00&.980\\
5&<0.05&<0.05&<0.05&1.00&1.00&1.00
&<0.05&<0.05&<0.05&\R{.200}&\R{.280}&1.00\\
6&<0.05&<0.05&<0.05&.650&1.00&.920&
<0.05&<0.05&<0.05&.690&1.00&.630\\
7&<0.05&<0.05&<0.05&.950&1.00&.970
&<0.05&<0.05&<0.05&\R{.530}&1.00&1.00\\
8&\R{0.46}&<0.05&<0.05&\R{.530}&1.00&.990
&<0.05&<0.05&<0.05&.810&1.00&1.00\\
9&<0.05&<0.05&\R{1.00}&.650&1.00&1.00
&<0.05&<0.05&\R{1.00}&.800&1.00&1.00\\
\hline
&\multicolumn{12}{c|}{\textbf{Coverage of target instructions}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.900&.990&.880
&<0.05&<0.05&<0.05&.660&.760&\R{.350}\\
2&<0.05&<0.05&<0.05&.620&.980&.560
&<0.05&<0.05&<0.05&.940&.980&\R{.200}\\
3&\R{0.81}&<0.05&<0.05&\R{.490}&1.00&.980
&<0.05&<0.05&<0.05&.960&1.00&.760\\
4&<0.05&<0.05&<0.05&.950&1.00&.940
&<0.05&<0.05&<0.05&.940&1.00&.980\\
5&<0.05&<0.05&<0.05&1.00&1.00&1.00
&<0.05&<0.05&<0.05&\R{.200}&\R{.280}&1.00\\
6&<0.05&<0.05&<0.05&.790&1.00&.610
&<0.05&<0.05&<0.05&.720&1.00&\R{.400}\\
7&<0.05&<0.05&<0.05&.970&1.00&.990
&<0.05&<0.05&<0.05&\R{.550}&1.00&1.00\\
8&<0.05&<0.05&<0.05&.660&1.00&.990
&<0.05&<0.05&<0.05&.900&1.00&1.00\\
9&\R{0.05}&<0.05&\R{1.00}&.680&1.00&.728
&<0.05&<0.05&\R{1.00}&.810&1.00&.656\\
\hline
\end{tabular}
\textbf{Legend}: \emph{C}, case study. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$ ) or no higher likelihood (i.e., $A_{12} < 0.56$) of covering more targets  than state-of-the-art approaches.
\end{table}%

